Causal Discovery of Dynamic Models for Predicting Human Spatial Interactions

Exploiting robots for activities in human-shared environments, whether warehouses, shopping centres or hospitals, calls for such robots to understand the underlying physical interactions between nearby agents and objects. In particular, modelling cause-and-effect relations between the latter can help to predict unobserved human behaviours and anticipate the outcome of specific robot interventions. In this paper, we propose an application of causal discovery methods to model human-robot spatial interactions, trying to understand human behaviours from real-world sensor data in two possible scenarios: humans interacting with the environment, and humans interacting with obstacles. New methods and practical solutions are discussed to exploit, for the first time, a state-of-the-art causal discovery algorithm in some challenging human environments, with potential application in many service robotics scenarios. To demonstrate the utility of the causal models obtained from real-world datasets, we present a comparison between causal and non-causal prediction approaches. Our results show that the causal model correctly captures the underlying interactions of the considered scenarios and improves its prediction accuracy.

==> approach.tex <==
\section{Causal discovery from observational data} \label{sec:appr}
Our approach is based on the observation of human spatial behaviours to recover the underlying SCM. This causal analysis is performed by using the PCMCI causal discovery algorithm \cite{runge_causal_2018}. First, we identify some important factors (i.e. variables) affecting human motion in the considered scenarios, and from that we reconstruct the most likely causal links from real sensor data. Finally, we use the discovered causal models to forecast the latter with a state-of-the-art Gaussian Process Regression (GPR) technique~\cite{rudenko2020human,li2020data}, showing that the causality-based GPR improves the accuracy of the human (interaction) prediction compared to a non-causal version.
%Since its flexibility and the little prior process knowledge requirement, GPR has become a popular tool for learning dynamic systems from data, widely used in robotics, especially in Human-Robot interaction \cite{li2020data}.
%The latter has become a popular tool for learning dynamic systems from data, since it is flexible, requires little prior process knowledge and inherently provides a measure of model uncertainty by providing a probabilistic distribution over function values.
%Moreover, it is widely used by the robotics community, especially in Human-Robot interaction \cite{li2020data}.
Two different scenarios have been modelled and analysed.

\begin{figure}[b]
\centering 
\subfloat{
    \label{fig:exp_thor}
    \includegraphics[width=0.32\columnwidth]{resource/thor.png}}
%\subfloat{
%    \label{fig:exp_atc}
%    \includegraphics[scale=0.4]{resource/exp_atc.png}}\\
\subfloat{
    \label{fig:approach_hg_scenario}    \includegraphics[width=0.32\columnwidth]{resource/approach_hg_scenario.eps}}
\subfloat{
    \label{fig:approach_hmo_scenario}
    \includegraphics[width=0.32\columnwidth]{resource/approach_hmo_scenario.eps}}
\vspace{-7pt}
\caption{\small{Image from TH{\"O}R dataset \cite{thorDataset2019} (left). Representation of the two analysed scenarios: (centre) the human-goal scenario, (right) the human-moving obstacles scenario. The agents consist of a circle and an arrow specifying, respectively, the current position and orientation. The selected agent is red, while, the obstacles are black.}}
\vspace{\negspace}
\label{fig:approach_scenarios}
\end{figure}

\subsection{Human-goal scenario} \label{subsec: Human-goal scenario}
Our first scenario includes interactions between human and (static) goals in a warehouse-like environment, illustrated in Fig.~\ref{fig:approach_scenarios}~(centre), where the agent walks among different positions (grey squares) to move some boxes or grab/use some tools. The grey line connecting agent and goal specifies the angle~$\theta_g$ between the two. Upon expert judgment, the following features were deemed essential to explain the human motion behaviour: \textit{(i)}~angle agent-goal $\theta_g$; \textit{(ii)}~euclidean distance agent-goal $d_g$; \textit{(iii)}~agent velocity $v$.
%\vspace{-5pt}
%\begin{itemize}
%    \item angle agent-goal $\theta_g$;
%    \item euclidean distance agent-goal $d_g$;
%    \item agent velocity $v$.
%\end{itemize}
%\vspace{-5pt}
The angle $\theta_g$ represents the human intention to reach a desired position (the person will first point towards the desired target before reaching it); then the person walks towards the goal, reducing the distance from it, at first by increasing the walking speed and finally decreasing, when closed to the destination. Soon after the human has reached the goal, $\theta_g$ changes to the next one, and the process restarts. %so it works like a trigger to change the target.
What we expect from this scenario are therefore the following causal relations:
\vspace{-5pt}
\begin{enumerate}[label=(\alph*)]
    \item $\theta_g$ depends on the distance, when the latter decreases to zero then $\theta_g$ changes;
    %\item $d_g$ depends on $\theta_g$, since when the latter changes it means that the human points a new target, and then the distance changes. Moreover, $d_g$ is inversely related to $v$;
    \item $d_g$ is inversely related to $v$ and depends on $\theta_g$;
    \item $v$ is a direct function of the distance $d_g$. 
\end{enumerate}
\vspace{-5pt}
\subsection{Human-moving obstacles scenario} \label{subsec: Human-moving obs scenario}
The second scenario involves multiple agents. It reproduces the interaction between a selected human and nearby dynamic obstacles (e.g. other humans, mobile robot), as shown in Fig.~\ref{fig:approach_scenarios}~(right). In this case, we take into account human reactions to possible collisions with obstacles, modelled by a \textit{risk} factor.
Consequently, the relevant features in this scenario are \textit{(i)}~euclidean distance~$d_g$ of the selected agent-goal, \textit{(ii)}~agent's velocity $v$, and \textit{(iii)}~\textit{risk} value.
%\vspace{-5pt}
%\begin{itemize}
%    \item euclidean distance selected agent-goal $d_g$;
%    \item selected agent velocity $v$;
%    \item \textit{risk} value.
%\end{itemize}
%\vspace{-5pt}
The agent moves between goals in the environment, so the cause-effect relation between distance and velocity will be similar to the previous scenario. The main difference in this case is that, instead of reaching the goal without problems, the agent needs to take into account the presence of other obstacles, and the interactions with them will affect the resulting behaviour. In particular, the agent's velocity is affected by possible collisions (e.g. sudden stop or direction change to avoid an obstacle). Hence, the expected causal links in this scenario are the following ones:
\vspace{-5pt}
\begin{enumerate}[label=(\alph*)]
    \item $d_g$ depends inversely on $v$;
    \item $v$ is a direct function of the $d_g$, but it is also affected by the collision $risk$;
    \item $risk$ depends on the velocity, as explained below.
\end{enumerate}
\textbf{Obstacle detection and risk evaluation:} in the literature, there are several strategies for identifying obstacles and evaluating the risk of collision with them. In order to model a numerical $risk$ value as a function of the agent's interactions, we implemented a popular strategy named Velocity Obstacles~(VO)~\cite{Fiorini1998}. The VO technique identifies an unsafe sub-set of velocities for the selected agent that would lead to a collision with a moving or static obstacle, assuming the latter maintains a constant velocity.

The risk can then be defined as follows. At each time step, we apply the VO strategy to the agent's closest obstacle. Such risk is a function of two parameters, both depending on the velocity of the selected agent (i.e. point $P$ inside the VO; see Fig.~\ref{fig:approach_velocity_obstacle}):
\vspace{-5pt}
\begin{itemize}
    \item $d_{OP}$, the distance between the cone's origin $O$ and $P$, which is proportional to the time available for the selected agent A to avoid the collision with B;
    \item $d_{BP}$, the distance between $P$ and the closest cone's boundary, which indicates the steering effort required by A to avoid the collision with B.
\end{itemize}
\vspace{-5pt}
Consequently, the risk of collision is defined as follows:
\begin{equation} \label{eq:risk}
risk = e^{d_{OP} + d_{BP} + v_a}.
\end{equation}
In order to avoid mostly-constant values (undetectable by the causal discovery algorithm), we introduced a third parameter $v_a$, which is the velocity of the selected agent. Therefore, the risk depends mainly on the agent's velocity, plus the VO's contributions in case of interaction with another agent.

\begin{figure}[t]\centering
\includegraphics[width=0.65\columnwidth]{resource/approach_velocity_obstacle.eps}
\caption{\small{Velocity Obstacle (VO) technique. The selected agent (A) and the obstacle (B) are shown in red and black, respectively. A Collision Cone (CC) is built from A to the enlarged encumbrance of B. Then, the CC is translated by $v_b$ to identify the VO, which partitions the velocity space of A into \textit{avoiding} and \textit{colliding} regions, i.e. velocities lying outside and inside the VO, respectively. The example on the left shows an interaction leading to a collision, since $v_a$ falls inside the VO. On the right, instead, is a collision-free interaction, since $v_a$ is outside the VO.}}
\vspace{\negspace}
\label{fig:approach_velocity_obstacle}
\end{figure}

\subsection{Causal prediction}
Our approach for modeling and predicting spatial interactions, shown in Fig.~\ref{fig:intro}, can be decomposed in three main steps: (\textit{i})~extract the necessary time-series of sensor data from the two previously explained scenarios; (\textit{ii})~use them for the causal discovery performed by the PCMCI algorithm; (\textit{iii})~finally, embed the causal models in a GPR-based prediction system.
More in detail, PCMCI is a causal discovery algorithm consists of two parts: the well-known PC algorithm, which starts from a fully connected graph and, by performing conditional independence tests, outputs an initial causal model structure; the latter is then used by the second part, the MCI test, which validates the structure by estimating the p-values and other test statistics for all the links. After that, we exploit the obtained causal model to predict with the GPR the value of each variable by using only its parents, and not all the variables involved in the scenario, as a non-causal GPR predictor would do.
%\begin{figure}[t]\centering
%\includegraphics[trim={0cm 3.6cm 0cm 3cm}, clip, width=\columnwidth]{resource/approach_causal_prediction.pdf}
%\vspace{-20pt}
%\caption{Causal prediction approach}
%\vspace{-20pt}
%\label{fig:approach_causal_prediction}
%\end{figure}
%\subsection{Simulation environment}
%To reproduce the human behaviours of the two previously mentioned scenarios we modelled the human as a unicycle. Since we are modelling a relatively slow walking person, a reasonable choice for the sampling frequency is $10Hz$.
%In order to guide the agents among the goals in the environment and to avoid the other agents, we used Artificial Potential Fields as motion planning technique \cite{Bemporad1996}.
%In particular, we used an attractive potential field to attract the agent to a desired position, plus a VO and repulsive potential field combination to keep the agent away from the obstacles in the environment. The selected agent is affected by the repulsive field only if it is inside the range of influence of the obstacle and a collision is detected by the VO strategy. Moreover, we derived the repulsive force in the vortex version to overcome the problem of local minima and to force the agent to circumvent the obstacles and not be repelled by them. In order to be as close as possible to a real scenario and to respect the \textit{faithfulness} causal assumption \cite{runge_causal_2018}, a synthetic gaussian noise have been added to the variables coming from the simulated environment, and then used for the causal analysis.


==> experiments.tex <==
\section{Experiments} \label{sec:exp}
We evaluated our approach for causal modeling and prediction of human spatial behaviours on two challenging datasets: TH{\"O}R~\cite{thorDataset2019} and ATC Pedestrian Tracking~\cite{brvsvcic2013person}. Both contains data of people moving in indoor environments, a workshop/warehouse and a shopping center, respectively. Our strategy is first to extract the necessary time-series from the two datasets, as explained in Sec.~\ref{sec:appr}, and then use it for causal discovery. In order to prove the usefulness of the causal models, a comparison between causal and a non-causal predictions is finally shown. %A Gaussian Process Regressor was used to forecast the observed timeseries leveraging the knowledge of the causal model structure. The results are then compared with the results of the forecasting performed without the causal models.
We considered two different datasets in order to verify, for the first scenario in Sec.~\ref{subsec: Human-goal scenario}, that the discovered causal model holds for similar human behaviours, even when observed in different environments. The scenario in Sec.~\ref{subsec: Human-moving obs scenario}, instead, is used to demonstrate that it is possible to perform causal discovery for other types of human spatial interactions (i.e. with collision avoidance).

\subsection{Data processing}
From both datasets, we extracted the $x$-$y$ positions of each agent and derived all the necessary quantities from them (i.e. orientation $\theta$, velocity $v$, etc.).\\
\textbf{TH{\"O}R dataset:} this provides a wide variety of interactions between humans, robot, and static objects~(Fig.~\ref{fig:approach_scenarios}~(left)). Helmets and infrared cameras were used to track the motion of the agents at~$100~Hz$. We used this dataset to analyse both scenarios (Sec.~\ref{subsec: Human-goal scenario} and Sec.~\ref{subsec: Human-moving obs scenario}). Moreover, to reduce the computational cost of causal discovery on this dataset, due to the large amount of samples in the time-series, we selected only a subset of them using an entropy-based adaptive-sampling strategy~\cite{Aldana-Bobadilla2015}, with an additional variable size windowing approach to reduce
the number of samples.\\
\textbf{ATC pedestrian tracking dataset:} in this case, the data was collected in the large atrium of a shopping mall (much bigger than TH{\"O}R's environment). Several 3D~range sensors were used to track people at $30~Hz$. Due to its large area and crowd, this dataset was not suitable for the collision-enhanced scenario in Sec.~\ref{subsec: Human-moving obs scenario}. Indeed, the large distance between humans and goals made the VO and the risk analysis difficult to estimate. Therefore, we used this dataset only for the scenario in Sec.~\ref{subsec: Human-goal scenario}, assuming that the interactions and collision avoidance between humans could be captured by the model's noise variance.

\subsection{Results}
We report the causal models discovered by PCMCI for the two scenarios. All the causal models were obtained using the same conditional independence test based on Gaussian Process regression and Distance Correlation (GPDC)~\cite{runge_detecting_2019}. We used also a 1-step lag time, that is, variables at time $t$ could only be affected by those at time $t-1$.
%
The resulting causal models are illustrated in Fig.~\ref{fig:exp_causal_model}, where the thickness of the node's border represents the variable's autocorrelation, while the arrows' thickness denote the strength of the causal links between different variables (the stronger the autocorrelation/causal link, the thicker the line). The number on each link/node specifies the lag time of the causal relation (always $1$ in this case).


\begin{figure*}[t]
\centering 
\subfloat{
    \includegraphics[trim={2.5cm 2cm 2.5cm 1.3cm}, clip, width=0.33\textwidth]{resource/exp_cm_hg_thor_dag.eps}}
\subfloat{
    \includegraphics[trim={2.5cm 2cm 2.5cm 1.3cm}, clip, width=0.33\textwidth]{resource/exp_cm_hg_atc_dag.eps}}
\subfloat{ 
    \includegraphics[trim={2.5cm 2cm 2.5cm 1.3cm}, clip, width=0.33\textwidth]{resource/exp_cm_hmo_thor_dag.eps}}
\vspace{-7pt}
\caption{\small{Causal models of human-goal scenario: (left) TH{\"O}R, (centre) ATC datasets. Causal model of human-moving obstacles scenario: (right) TH{\"O}R dataset.}}
\vspace{\negspace}
\label{fig:exp_causal_model}
\end{figure*}

In particular, Fig.~\ref{fig:exp_causal_model} shows the causal models of the human-goal~(left and centre) and the human-moving obstacles scenarios~(right). All the three graphs agree with the expected models discussed in Sec.~\ref{subsec: Human-goal scenario} and Sec.~\ref{subsec: Human-moving obs scenario}. This confirms that the same causal structure in the first two graphs generalises to similar human behaviours in different datasets, although autocorrelations and causal strengths vary between them due to different sampling frequencies and noise levels. The third graph demonstrate that it is possible to obtaining different causal models for different human behaviours.

%The \textit{significance level} parameter\todo{\textbf{Question}\\Should I leave this part about $\alpha$?}, $\alpha$, plays an important role by setting the false positive rate threshold, which determines if a link between two nodes can be maintained or removed based on its p-value. %In order to identify the correct value of $\alpha$ for each scenario, we exploited the Structural Hamming Distance (SHD) metric \cite{DeJongh2009} to compare, for different values of $\alpha$, the causal graphs from the real datasets to those obtained from the simulations. The SHD is a simple metric which counts the difference in terms of number of edges to compare two causal graphs. To evaluate our approach we performed the causal analysis starting with $\alpha$ equal to $0.05$ (i.e. max false positive rate 5\%) and then we tuned it to obtain the best results (knowing the ground-truth causal models).

%\begin{figure}[t]\centering
%\includegraphics[width=0.75\columnwidth]{resource/exp_shd.eps}
%\caption{Structural Hamming distance analysis. (a) and (b) SHD Human-goal scenario using TH{\"O}R  and ATC, respectively; (c) SHD Human-moving obstacles scenario using TH{\"O}R}
%\label{fig:exp_shd}
%\end{figure}


%\begin{figure}[t]
%\centering
%\subfloat{
%    \label{fig:exp_simulation_interaction}
%    \includegraphics[trim={2.5cm 2cm 2.5cm 1.3cm}, clip, width=0.43\textwidth]{resource/exp_cm_hmo_sim_dag.eps}}
%\subfloat{
%    \label{fig:exp_thor_interaction}    
%    \includegraphics[trim={2.5cm 2cm 2.5cm 1.3cm}, clip, width=0.43\textwidth]{resource/exp_cm_hmo_thor_dag.eps}}
%    \vspace{-5pt}
%\caption{Causal model of human-obstacle scenario: (left) simulated data, (right) TH{\"O}R dataset. The causal models structure from the dataset (right) and the ground-truth (left) coincides.}
%\label{fig:exp_hmo}
%\end{figure}
%Fig. \ref{fig:exp_shd} shows the SHD analysis on the three causal graphs from the datasets, with $\alpha$ varying in the range $[0.001, 0.05]$. In particular, the blue line identifies the SHD of the causal graph coming from TH{\"O}R with respect to the ground-truth in the Human-goal scenario. It highlights that for a small range of $\alpha$ values, we can get the same DAG. The red line represents the SHD on the same scenario but using the ATC dataset and, in this case, we can observe that the causal model is more robust than the previous one, since it maintains the SHD equals to zero for a large range of $\alpha$ values. Then, for $\alpha < 2\%$ the SHD increases. Finally, the yellow line shows the SHD for the Human-moving obstacles scenario using TH{\"O}R with respect to the ground-truth and, again, the SHD analysis helped to find a correct range for $\alpha$. \todo{taken from the PhD transfer. Is it ok to have it here too?}\textcolor{red}{Note that, even if for some $\alpha$ values the causal graphs result different to the ground-truth, the SHD remains always relatively small across the full range of $\alpha$ values. Indeed, the maximum SHD obtained from the experiments is $3$, against the maximum possible SHD $=9$ (for this particular application). Moreover, from Fig.~\ref{fig:exp_shd}, it is clear that by selecting a common $\alpha$ value for all scenarios such that $0.02 \le \alpha \le 0.022$, the worst-case SHD is only $1$.}




%Fig.~\ref{fig:exp_causal_model}~(left and centre) show the two causal models for the Human-goal scenario. By properly tuning the PCMCI algorithm, the two results have exactly the same structure, in accordance with the expected structure discussed in Sec.~\ref{subsec: Human-goal scenario}. \textcolor{red}{This confirms the concept of obtaining the same causal graph when we are observing the same behaviour, even from different datasets.}
%Moreover, due to the different sampling frequencies and levels of noise in the datasets, we can observe different auto- and cross-dependency relationship strength between the two graphs. The same considerations hold for the result of the Human-moving obstacle scenario in Fig.~\ref{fig:exp_causal_model}(right). In fact, also in this case, \textcolor{red}{by selecting the best value of $\alpha$}, the result from the real dataset agrees with the expected structure discussed in Sec.~\ref{subsec: Human-moving obs scenario}. \textcolor{red}{Note that this result confirms the concept of obtaining different causal graphs when we are observing different behaviours, even from the same dataset.}

\begin{figure*}[t]
\centering 
\subfloat{
    \label{fig:exp_pred_cNRMSE_theta}
    \includegraphics[trim={1.2cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_thetag_cNRMSE.eps}}
\subfloat{
    \label{fig:exp_pred_cNRMSE_d}
    \includegraphics[trim={1.2cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_dg_cNRMSE.eps}}
\subfloat{
    \label{fig:exp_pred_cNRMSE_v}
    \includegraphics[trim={0.9cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_v_cNRMSE.eps}}\\
    \vspace{-10pt}
\subfloat{
    \label{fig:exp_pred_ncNRMSE_theta}
    \includegraphics[trim={1.2cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_thetag_ncNRMSE.eps}}
\subfloat{
    \label{fig:exp_pred_ncNRMSE_d}
    \includegraphics[trim={1.2cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_dg_ncNRMSE.eps}}
\subfloat{
    \label{fig:exp_pred_ncNRMSE_v}
    \includegraphics[trim={0.9cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_v_ncNRMSE.eps}}\\
    \vspace{-10pt}
\subfloat{
    \label{fig:exp_pred_theta}
    \includegraphics[trim={1.2cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_thetag_pred.eps}}
\subfloat{
    \label{fig:exp_pred_d}
    \includegraphics[trim={1.2cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_dg_pred.eps}}
\subfloat{
    \label{fig:exp_pred_v}
    \includegraphics[trim={0.9cm 0.6cm 2cm 1cm}, clip, width=0.32\textwidth]{resource/exp_pred_hg_thor_v_pred.eps}}
\vspace{-7pt}
\caption{\small{Time-series prediction on the human-goal scenario of the TH{\"O}R dataset for the spatial interaction variables $\theta_g$~(left), $d_g$~(centre), $v$~(right). (Top line) NRMSE of the prediction using the causal model. (Central line) NRMSE of the prediction with no causal model. (Bottom line) Examples of predicted time-series.
}}
\vspace{\negspace}
\label{fig:exp_pred}
\end{figure*}

The obtained causal models are then exploited for the prediction of the spatial interaction variables in both scenarios. For example, in case of the human-goal scenario using the TH{\"O}R dataset, the prediction of $\theta_g$ was done using only its parent $d_g$ in the respective causal model (Fig.~\ref{fig:exp_causal_model}, left). To evaluate the advantage of using our models, we benchmarked the prediction performance with a causally-informed GPR estimator against a non-causal one, where the latter considers all the variables possibly influencing each other. Fig.~\ref{fig:exp_pred} shows the comparison between causal and non-causal prediction for the human-goal scenario with the TH{\"O}R dataset, using the \textit{Normalised Root Mean Square Error} (NRMSE) as evaluation metric. The figure shows that our causal model helps to predict the time-series more accurately compared to the non-causal case. Indeed, the NRMSE of the causal predictor (Fig.~\ref{fig:exp_pred}, top line) is lower than the non-causal one (Fig.~\ref{fig:exp_pred}, central line) for all the variables. Moreover, the graphs at the bottom show some examples where the time-series predicted using our causal model (orange line) are always closer to the ground-truth (blue line) than those predicted without it (green line). Finally, Table~\ref{tab:exp_NRMSE} summarises the prediction results for all the considered scenario, clearly showing that the causal prediction approach outperforms always the non-causal one. Note that, for the human-goal scenario, the NRMSE in the ATC dataset are bigger than in TH{\"O}R, which is probably due to the different time-series lengths in the two datasets.

\begin{table*}[t]
\begin{center}
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\begin{tabular}{l||ccccccccc|}
           & \multicolumn{6}{c|}{Human-goal}                                                                                                    & \multicolumn{3}{c|}{Human-moving obs}  \\ \cline{2-10} 
           & \multicolumn{3}{c|}{TH{\"O}R}                                   & \multicolumn{3}{c|}{ATC}                                     & \multicolumn{3}{c|}{TH{\"O}R} \\ \cline{2-10} 
           & \theta_g & d_g & \multicolumn{1}{c|}{v}    & \theta_g & d_g  & \multicolumn{1}{c|}{v}    & d_g    & v      & risk   \\ \hline
Causal     & \textbf{0.32}                     & \textbf{0.37} & \multicolumn{1}{c|}{\textbf{0.08}} & \textbf{2.4}                      & \textbf{1.8}   & \multicolumn{1}{c|}{\textbf{0.25}} & \textbf{0.11}    & \textbf{0.25}   & \textbf{0.34}   \\
Non-causal & 1.35                     & 5.54 & \multicolumn{1}{c|}{1.42} & 9.15                     & 29.03 & \multicolumn{1}{c|}{1.04} & 4.8     & 1.04   & 3.96   \\ \hline
\end{tabular}
\end{center}
\vspace{-7pt}
\caption{\small{NRMSE of causal and non-causal predictions for both scenarios and datasets.}}
\vspace{\negspace}
\label{tab:exp_NRMSE}
\end{table*}

==> related_work.tex <==
\section{Related work} \label{sec:related}

%Human-Robot Spatial Interaction
\textbf{Human Spatial Interaction} Dynamic Bayesian Networks (DBNs), Deep recurrent models, QTC, etc.

%Causal discovery
\textbf{Causal Discovery} Structural causal models (SCMs) form the basis for our research \cite{alma991011292629705181} and can be explained by the Directed Acyclic Graphs (DAGs), composed by nodes and oriented edges to represent respectively, variables and oriented dependencies between them (see Fig. \ref{fig:intro}). The knowledge of SCMs leads to the possibility to reason on the cause-and-effect relationship between variables. 

Several methods have been developed over the last few decades to derive causal models from observational data. They can be categorised into two main classes, reviewed in \cite{glymour_review_2019}. The first, constraint-based methods, such as Peter and Clark (PC) and Fast Causal Inference (FCI) use conditional independence tests to recover the causal graph, while the second, score-based methods, such as Greedy Equivalence Search (GES) assign a score to each DAG, and perform searching in this score space. Recently, reinforcement learning-based method has been used to discover causal structure \cite{Zhu2019}. Further, causal discovery from a mix of observational and interventional data has been studied in \cite{Gasse2021,ke_learning_2019}.

However, many of those algorithms work only with static data (i.e. temporal order not considered) and this may represent a problem for robotics applications.
In fact, time-dependent causal discovery methods come to the rescue when we are dealing with an application where the temporal order of the data is required to recover the correct behaviour of the system. %Their use implies the need to modify some basic notations such as DAGs, shown in Fig. \ref{fig:causal_timeseries}.
In \cite{runge_causal_2018}, a variation of the PC algorithm adapted to time series data is introduced. This method, called PCMCI, is designed to efficiently reconstruct causal graphs from high-dimensional timeseries datasets with an additional optimisation regarding the control of the false positive rate, performed by the momentary conditional independence (MCI) test. %An extension of the PCMCI algorithm, called PCMCI\textsuperscript{+}, has been introduced in \cite{runge2020discovering}, to include discovery of contemporaneous links.

\textbf{Causal discovery applications}
%Causal discovery applications
In \cite{runge_detecting_2019,saetia_constructing_2021}, we can find applications of it in climate and healthcare sectors. Causal discovery method finds space also in the machine learning field \cite{scholkopf_toward_2021,Seitzer2021} where the authors review basic concepts of causal inference and relate them to crucial open problems of machine learning, discussing how they can benefit for the causal inference introduction. %They discuss the fact that most RL algorithms do not explicitly consider the relations between entities in the environment and propose to integrate causal inference into RL algorithms to improve exploration and to assist the policy learning.

Some applications of causal discovery methods can be found in the robotics field. 
% A causal approach to tool affordance learning
In \cite{brawer_causal_2021} a method has been introduced for a robot to learn an explicit model of cause-and-effect by constructing a structural causal model through a mix of observation, using PC algorithm, and self-supervised experimentation. Then, this method has been demonstrated on tool affordance tasks where a humanoid robot had to leverage its prior learning to utilise novel tools effectively.
% Reasoning Operational Decisions for Robots via Time Series Causal Inference
Another application in the robotics field is presented in \cite{cao_reasoning_2021} where the PCMCI algorithm has been used to derive the causal model of an underwater robot reaching a target position. Reasoning on it enables the robot to predict how its actions will affect the distance to the goal.
% A novel parsimonious cause-effect reasoning algorithm for robot imitation and plan recognition
In \cite{Katz2018,Angelov2019}, two imitation learning applications can be found. In \cite{Katz2018} the authors wanted to replicate the same approach of imitation learning in people; indeed, their approach constructs an explanation for a demonstrator's actions and then generates a plan to carry out the same goal, rather than faithfully reproducing the demonstrator’s actions.
% Using causal analysis to learn specifications from task demonstrations
In \cite{Angelov2019}, causal analysis has been used to classify human behaviours from demonstrations, highlighting the comparison between results from observational and intervational data.

% Highlight contributions
\textcolor{red}{Nevertheless, none of the above applications exploit causality to better understand the Human Spatial Interaction (including HRSI), as we aim in this paper. In fact, our goal is to use causal analysis to make the robot understand possible human motion behaviours, from the spatial point of view, when they collaborate and share the same environment. Our work represents the first step toward that direction, which is, leveraging a causal discovery method to reconstruct the model behind human spatial behaviours. To this end, we will create some causal models of typical human spatial interaction in some challenging setting.}



